AMReX: Block-Structured Adaptive Mesh Refinement for Multiphysics Applications

Block-structured adaptive mesh refinement (AMR) provides the basis for the temporal and spatial discretization strategy for a number of ECP applications in the areas of accelerator design, additive manufacturing, astrophysics, combustion, cosmology, multiphase flow, and wind plant modelling. AMReX is a software framework that provides a unified infrastructure with the functionality needed for these and other AMR applications to be able to effectively and efficiently utilize machines from laptops to exascale architectures. AMR reduces the computational cost and memory footprint compared to a uniform mesh while preserving accurate descriptions of different physical processes in complex multi-physics algorithms. AMReX supports algorithms that solve systems of partial differential equations (PDEs) in simple or complex geometries, and those that use particles and/or particle-mesh operations to represent component physical processes. In this paper, we will discuss the core elements of the AMReX framework such as data containers and iterators as well as several specialized operations to meet the needs of the application projects. In addition we will highlight the strategy that the AMReX team is pursuing to achieve highly performant code across a range of accelerator-based architectures for a variety of different applications.

==> intro_save.tex <==
AMReX, a software framework developed and supported by the DOE Exascale Computing Program's AMR Co-Design Center, supports the development of block-structured adaptive mesh refinement (AMR) algorithms for solving systems of partial differential equations, in simple or complex geometries, on exascale architectures. Block-structured AMR provides the basis for the temporal and spatial discretization strategy for a large number of ECP applications in the areas of accelerator design, astrophysics, combustion, cosmology, multiphase flow, additive manufacturing and wind energy. \MarginPar{ExAM} 
AMReX provides a unified infrastructure with the functionality needed for these and other AMR applications to be able to effectively utilize exascale architectures. AMR reduces the computational cost and memory footprint compared to a uniform mesh while preserving the local descriptions of different physical processes in complex multi-physics algorithms. 

AMReX supports algorithms that utilize particles and/or particle-mesh operations to represent component physical processes in addition to mesh-based solution approaches.  Fundamental to block-structured AMR algorithms is a hierarchical representation of the solution at multiple levels of resolution. At each level of refinement, the solution is defined on the union of data containers at that resolution, each of which represents the solution over a logically rectangular subregion of the domain. Solution strategies vary from level-by-level approaches (with or without subcycling in time) with multilevel synchronization to full-hierarchy approaches, and any combination thereof. AMReX provides data containers and iterators that understand the underlying hierarchical parallelism for field variables on a mesh, particle data and embedded boundary (cut cell) representations of complex geometries. Both particles and embedded boundary representations introduce additional irregularity and complexity in the way data is stored and operated on, requiring special attention in the presence of the dynamically changing hierarchical mesh structure and AMR time stepping approaches.  AMReX also provides performance portability, enabling AMReX-based applications to move between CPU-based architectures and different hybrid CPU-accelerator systems with minimal changes to the application code itself.

Additional text at
https://www.exascaleproject.org/amrex-co-design-center-helps-five-application-projects-reach-performance-goals

==> regridding.tex <==
\subsubsection{Regridding and load balancing}
\label{sec:regrid}

AMR algorithms dynamically change the resolution of the mesh to reflect the changing requirements of the problem being solved.  
AMReX provides support for the creation of new grids or the modification of existing grids (regridding) at level $\ell+1$ and above at user-specified intervals. To do so, 
\commentout{Given data at level $\ell-1$}
an error estimate is used to tag individual cells above a given tolerance at level $\ell$, where the error is defined by user-specified routines.  Typical error criteria might include,
first or second derivatives of the state variables or some type of application-specific heuristic.

The tagged cells are grouped into rectangular grids at level $\ell$ using the clustering algorithm given in \cite{bergerRigoutsos:1991}.
These rectangular patches are refined to form the grids at level $\ell+1$.
Large patches are broken into smaller patches for distribution to multiple 
processors based on a user-specified \texttt{max\_grid\_size} parameter; AMReX enforces that no grid is longer in any direction than \texttt{max\_grid\_size} cells.
AMReX also provides the option to enforce that the dimensions of each newly created grid is divisible by a specific factor, \texttt{blocking\_factor}; this is used to improve multigrid efficiency for single-level solves. (In this case the grid creation algorithm is slightly different; we refer the interested reader to the AMReX documentation: \cite{AMREX:2019,AMREX:Docs}.)
The refinement process is repeated until either an error tolerance criterion is satisfied or a specified maximum level is reached.  
Finally, we impose the proper nesting requirements that enforce that level $\ell+1$ is strictly contained in level $\ell$ except at physical boundaries.
A similar procedure is used to generate the initial grid hierarchy.
Once created, the \texttt{BoxArray} of new grids at each level is broadcast to every MPI rank.

\commentout{Once the new grids have been created, the new grid hierarchy needs to be distributed to the MPI ranks.}
%Load-balancing is so critical to AMR codes that even initial data distributions implement a default strategy.

When creating a \texttt{DistributionMapping} associated with a \texttt{BoxArray} at a level it is important to equidistribute the work to the nodes. Some type of cost function that is assumed or prescribed by the user is used to estimate the work.  The default methodology assumes a cost function proportional to the number of cells per grid, and implements a Morton-ordering space filling curve (SFC) algorithm to define an initial data distribution across the MPI ranks.
Once data has been allocated, applications can calculate an improved \texttt{DistributionMapping} throughout runtime based on any desired load-balancing parameter, such as data size, an estimation of the work, a user-defined cost function or a timer.

Prescribed cost functions are often less than optimal.  For GPUs, both CUPTI timers and efficient hand-written timers have been developed to accurately capture device kernel times respective to the device.  This eliminates launch delays and other latencies from the resulting timer that prevent accurate distribution.
  
AMReX provides a knapsack algorithm in addition to a space-filling curve algorithm for load balancing simulations across MPI ranks.  The knapsack algorithm creates the most optimal distribution possible with respect to the load-balancing parameter, while the SFC tries to build contiguous spatial regions with near uniform costs.  See Figure \ref{fig:load} for an illustration of how the two approaches distribute data.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{LoadBalancing.png}
    \caption{Comparison of the data distribution from the knapsack load balancing algorithm (left) and SFC (right).  Image courtesy of Michael Rowan.}
    \label{fig:load}
\end{figure}
\commentout{Once a new distribution mapping has been calculated, a simple call, the new distributed data containers can be filled from the old hierarchy.}
%\MarginPar{not sure i follow the last bit here.  tradeoff is buffering versus frequency.  also say something about how to fill in data}
%\MarginPar{Have a recent picture from Micheal Rowan's upcoming SC paper showing the difference between SFC and knapsack, if desired. It's uploaded as "LoadBalancing.png".}
%to \texttt{Redistribute} implements the calculated data mapping.  Load balancing can be expensive for large simulations, so characteristics like how often a new distribution is generated and the amount of improvement needed to trigger a redistribution must be tuned to provide optimal performance.

